Scheduling Drone and Mobile Charger via Hybrid-Action Deep Reinforcement Learning

Recently there has been a growing interest in industry and academia, regarding the use of wireless chargers to prolong the operational longevity of unmanned aerial vehicles (commonly knowns as drones). In this paper we consider a charger-assisted drone application: a drone is deployed to observe a set points of interest, while a charger can move to recharge the drone's battery. We focus on the route and charging schedule of the drone and the mobile charger, to obtain high observation utility with the shortest possible time, while ensuring the drone remains operational during task execution. Essentially, this proposed drone-charger scheduling problem is a multi-stage decision-making process, in which the drone and the mobile charger act as two agents who cooperate to finish a task. The discrete-continuous hybrid action space of the two agents poses a significant challenge in our problem. To address this issue, we present a hybrid-action deep reinforcement learning framework, called HaDMC, which uses a standard policy learning algorithm to generate latent continuous actions. Motivated by representation learning, we specifically design and train an action decoder. It involves two pipelines to convert the latent continuous actions into original discrete and continuous actions, by which the drone and the charger can directly interact with environment. We embed a mutual learning scheme in model training, emphasizing the collaborative rather than individual actions. We conduct extensive numerical experiments to evaluate HaDMC and compare it with state-of-the-art deep reinforcement learning approaches. The experimental results show the effectiveness and efficiency of our solution.

==> temp.tex <==
%%======================================================
\subsection{Reward Function}

In our model, the reward function $r(s,a)$ guides the drone and the charger to select suitable actions $a$ based on a given state $s$, aimed at maximizing the objective defined in \eqref{objective}. 
%%%%%%
As given below, this reward function exhibits four different forms under four types of actions. 

\emph{Reward for Observation} ($r^{\rm obs}$). When the drone decides to fly to observer $p_{i}$, \tbd 

%When drone flies to observe the $p_{i}$, we want to collect information as much as possible and shorten $t_{i, i+1}$. Meanwhile, we want to the charger goes to $c_j$ which nears the $p_{i}$ and $p_{i+1}$. Moreover, we add number of PoI to reward function as weight to encourage the drone to visit the next PoI.

\begin{equation}\label{r_obs}
r^{\rm obs} = i \cdot \frac{\sum_{p_i\in P}\,\nu_i(t_i^{\rm{obs}})}{\sum_{k \leq i}\, t_{k-1, k}} \cdot \frac{\{ \min(t^{\rm obs}, \tau^{\rm{max}}) + \frac{\rm{c}_1}{t_{i,j}\cdot t_{i+1, j}}\} }{t_{i-1, i}}
\end{equation}

\emph{Reward for Charging} ($r^{\rm chg}$).  

% When drone chooses the next charging point $c_{j}$, we hope the leave energy of drone denoted by $e_{j}$ in the $c_{j}$ is as few as possible and the recharged energy is full. Meantime, we hope $t^{\rm fly}_{i+1, j}$ and the minimum between $t^{\rm fly}_{i, j}$ and $\tau^{\rm chg}_{j}$ are as short as possible. Moreover, we add number of PoI to reward function as weight to encourage the drone to visit the next PoI. 

\begin{equation}
\label{r^{chg}}
r^{\rm chg} = i \cdot \frac{\sum_{p_i\in P}\,\nu_i(t_i^{\rm{obs}})}{\sum_{k \leq i}\, t_{k-1, k}} \cdot \frac{\min(t^{\rm chg}, \frac{\bf{e} - e_{j}}{\gamma_{c}})}{e_{j}\cdot \{ \max (t^{\rm fly}_{i, j}, \tau^{\rm chg}_{j} ) + t^{\rm fly}_{i+1, j} \} }
\end{equation}

\emph{Reward or Penalty for Task Failure} ($r^{\rm f}$). 

\begin{equation}
\label{r^{f}}
r^{\rm f} = - {\rm{c}_2} \cdot \sum_{p_i\in P}\frac{\tau^{\rm{max}}_i - t^{\rm{obs}}_i}{\tau^{\rm{max}}_i}\quad 
\end{equation}


% When the drone fails because of empty energy, we give it penalty according to the collected information and we hope it collects more information.

\emph{Reward for Task Completion} ($r^{\rm s}$).

% When the drone finishes its observation task and return the depot, we give it final reward considering of objective.



\begin{equation}
\label{r^{s}}
r^{\rm s} = {\rm{c}_3} \cdot \frac{\sum_{p_i\in P}\,\beta_i\cdot\nu_i(t_i^{\rm{obs}})}{t(\mathcal{E})}\quad 
\end{equation}

Above all, our reward function is:

\begin{equation}
\label{drone discrete action}
r(s,a) =\left\{
\begin{aligned}
& r^{\rm obs} & \mbox{observing}\\
& r^{\rm chg} & \mbox{charging}\\
& r^{\rm f} & \mbox{fail} \\
& r^{\rm s} & \mbox{success}
\end{aligned}
\right.
\end{equation}

Parameter ${\rm{c}_1}, {\rm{c}_2}, {\rm{c}_3}$ are the weight for different reward type.

\section{Deep RL-based Solution}\label{sec:design}

In this section, we first give a brief introduction to our \tbd and why ...\tbd , we then detail the designs of \ourModel, followed by the optimization algorithm that efficiently completes \ourModel training.
